Graphs for deep learning representations

In recent years, Deep Learning methods have achieved state of the art performance in a vast range of machine learning tasks, including image classification and multilingual automatic text translation. These architectures are trained to solve machine learning tasks in an end-to-end fashion. In order to reach top-tier performance, these architectures often require a very large number of trainable parameters. There are multiple undesirable consequences, and in order to tackle these issues, it is desired to be able to open the black boxes of deep learning architectures. Problematically, doing so is difficult due to the high dimensionality of representations and the stochasticity of the training process. In this thesis, we investigate these architectures by introducing a graph formalism based on the recent advances in Graph Signal Processing (GSP). Namely, we use graphs to represent the latent spaces of deep neural networks. We showcase that this graph formalism allows us to answer various questions including: ensuring generalization abilities, reducing the amount of arbitrary choices in the design of the learning process, improving robustness to small perturbations added to the inputs, and reducing computational complexity

==> X.tex <==
\def \tikzexternallastkey {07FDFDC8AC7EF80F9D76A863F39F5D5B}%


==> article_grellier.tex <==
\section{Bridging the gap between GFT and FT in Euclidean spaces}

In the previous Sections we have described how to extract graphs from data and from Euclidean structures and also defined the GFT and its inspiration from the ring graph and the Fourier Transform defined on an 1D Euclidean structure. However, when considering regular graphs of higher intrinsic dimension, this relationship between GFT and FT diverges. In this Section we detail our contributions from~\citep{grelier2018graph}, where we define an embedding function to convert graphs to Euclidean representations in order to match the GFT of the graph and the Fourier transform on the underlying Euclidean space.

To this end, we proposed the following methodology, taking as inputs a graph $G$ and an integer $d$:
\begin{enumerate}
\item Project vertices of the graph to $\mathbb{Z}^d$, such that geodesic distances between vertices in the graph are close to Manhattan distance between their projections in $\mathbb{Z}^d$,
\item Define GFT on $G$ as a particularization of the usual multidimensional FT on $\mathbb{Z}^d$.
\end{enumerate}
Obviously we expect this method to perform particularly well when facing approximations of (regular) grid graphs.

In the following subsections, we first introduce the problem statement for step~1 and initial results, we then show that this method guarantees that a 2D grid graph projection is exactly a rectangle in $\mathbb{Z}^2$, and that it is robust to minor changes in the graph structure. Finally, we introduce an optimization method for solving step~1 and perform experiments to compare with other embedding methods.

\subsection{Problem statement}

First, consider a weighted graph $\gG = \langle \sV, \sE \rangle$.

\begin{definition}[embedding]\label{chap3:def-embedding}
    We call \textbf{embedding} a function $\phi: \sV \to \mathbb{Z}^d$, where $d\in \mathbb{N}^*$.
\end{definition}

We are specifically interested in embeddings that preserve distances. Specifically, we define the cost $c_\alpha(\phi)$ of an embedding $\phi$ as the following quantity:
\begin{equation}
  c_\alpha(\phi) \triangleq \sum_{v,v' \in \sV}{| \; \alpha\|\phi(v) - \phi(v')\|_1 - d_\gG(v,v') \;|}\;,
\end{equation}
where $d_\gG$ is the shortest path distance in $\gG$. In the remaining of this Section, we denote $\delta(v,v') = | \; \alpha\|\phi(v) - \phi(v')\|_1 - d_\gG(v,v') \; |$.

\begin{definition}[optimal embedding]\label{chap3:def-optimalembedding}
    Given a fixed value of $\alpha$, we call \emph{optimal embedding} an embedding with minimum cost.
\end{definition}

Let us motivate the choices in this definition:
\begin{enumerate}
\item We consider all pairs of vertices and not only edges. Consider for example a ring graph where each vertex has exactly two neighbors. Then there are plenty of embeddings that would minimize the cost if considering only edges, but only a few that minimize the sum over all pairs of vertices.
\item We use a sum and not a maximum. This is because small perturbations of grid graphs would lead to dramatic changes in embeddings minimizing the cost if using a maximum. Consider for instance a 2D grid graph in which an arbitrary edge is removed.
\item We choose embedding in $\mathbb{Z}^d$ instead of in $\mathbb{R}^d$, as we want to particularize multidimensional \emph{discrete} Fourier transforms.
\item We use the Manhattan distance, as it is more naturally associated with $\mathbb{Z}^d$ than the Euclidean distance. It also ensures there exists natural embeddings for grid graphs with cost 0.
\item Finally, $\alpha$ is a scaling factor.
\end{enumerate}

Note that the question of finding suitable embeddings for graphs is not novel~\citep{Kobourov04forcedirecteddrawing}. But to our knowledge enforcing the embedding to be in $\mathbb{Z}^d$ is a novel contribution. Even though Definitions~\ref{chap3:def-embedding} and~\ref{chap3:def-optimalembedding} work for any $d$ we are going to focus on the consistency of these definitions by considering the particular case $d=2$, i.e., a regular 2D Euclidean space.

\begin{definition}[natural embedding]
    We call \emph{natural embedding} of a grid graph (as defined in Definition~\ref{chap3:def-gridgraph}) the identity function.
\end{definition}

A first interesting result is related to optimal embeddings of grid graphs.

\begin{theorem}
  The natural embedding of a grid graph is its only optimal embedding for $\alpha=1$, up to rotation, translation and symmetry.
  \label{chap3:theorem-grid}
\end{theorem}
\begin{proof}
  The proof is straightforward, as the cost of the natural embedding is clearly 0. Reciprocally, a cost of 0 forces any group of vertices $\{(x,y),(x,y'),(x',y),(x',y')\}$ to be projected to a translation, rotation and/or symmetry of the corresponding rectangle in $\mathbb{Z}^2$. Then any remaining vertex is uniquely defined from these four ones.
\end{proof}

\subsection{Robustness to small perturbation of grid graphs}

In this section we are interested in showing that the optimal embedding is robust to small perturbations of grid graphs. Here, we always consider $\alpha=1$. Let us first introduce quasi grid graphs as grid graphs with one missing edge:

\begin{definition}[quasi grid graph]
  A \emph{quasi grid graph} is a grid graph with one missing edge between vertices $(i,j)$ and $(i+1,j)$, with $1\leq i<\ell$ and $1< j< \ell$.
\end{definition}

We first prove results on two-slices graphs which is illustrated on Figure~\ref{chap3:fig-two-slices}:

\begin{definition}[two-slices graph]
  We call \emph{two-slices graph} a weighted graph with vertices of $\{1,2,3\} \times \{1,h\}$, where $h\geq 2$. It contains four weight-1 edges between vertices at Manhattan distance 1 from each other, and two weight-$h$ edges between vertices on the corner. We call natural embedding of a two-slices graph the identity function on its vertices.
\end{definition}

\begin{figure}[ht]
  \begin{center}
    \inputtikz{chapter3/tikz/two-slices}
  \end{center}
  \caption{Depiction of a two-slices graph. Figure extracted from~\citep{grelier2018graph}.}
  \label{chap3:fig-two-slices}
\end{figure}

First observe that the natural embedding of a two-slices graph has a cost of $4$.

\begin{lemma}
  Consider an embedding $\phi$ of a two-slices graph for which $\|\phi((2,1)) - \phi((2,h))\|_1\geq h + 4$, then $c_1(\phi) \geq 6$.
  \label{lemma1}
\end{lemma}
\begin{proof}
  It holds that $c_1(\phi) \geq 2\delta((2,1),(2,h)) + 2\delta((1,1),(2,h)) + 2\delta((1,1),(2,1))$. In particular the first term of the sum is at least $4$. Then we discuss two cases: a) $\delta((1,1), (2,1))\geq 1$ in which case the result is immediate or b) $\delta((1,1), (2,1)) \leq 1$ in which case the Manhattan distance between $(1,1)$ and $(1,h)$ is at least 3.
\end{proof}

\begin{lemma}
  Consider an embedding $\phi$ of a two-slices graph for which $\|\phi((2,1)) - \phi((2,h))\|_1 = h + 3$, then $c_1(\phi) \geq 8$.
  \label{lemma2}
\end{lemma}
\begin{proof}
  Again, we look at the vertex $(1,1)$. Either $\delta((1,1), (2,1))\geq 1$ or $(1,1)$ is at distance at least $h+2$ from $(2,h)$. In both cases, we obtain $\delta((1,1),(2,1)) + \delta((1,1), (2,h)) \geq 1$. We repeat the process for the other three vertices $(1,h), (3,h)$ and $(3,1)$.
\end{proof}

\begin{lemma}
  Consider an embedding $\phi$ of a two-slices graph for which $\|\phi((2,1)) - \phi((2,h))\|_1 = h + 2$, then $c_1(\phi) \geq 8$.
  \label{lemma3}
\end{lemma}
\begin{proof}
  Denote $v$ one of the four border vertices ($(1,1), (1,h), (3,1)$ or $(3,h)$). Either a) $\delta(v,(2,1)) = \delta(v,(2,h)) = 0$, or b) $\delta(v,(2,1)) + \delta(v,(2,h)) \geq 2$. Indeed, either $v$ is on a shortest (Manhattan) path between $(2,1)$ and $(2,h)$, or it is not. If two of the border vertices verify b) the proof is finished. If only one verifies b), then one of the following holds: i) $\|\phi((1,1)) - \phi((3,h))\|_1 = h$ or ii) $\|\phi((3,1)) - \phi((1,h))\|_1 = h$. In both cases we conclude. Finally, if all border vertices are in case a), then both i) and ii) hold.
\end{proof}

\begin{lemma}
  Consider an embedding $\phi$ of a two-slices graph for which $\|\phi((2,1)) - \phi((2,h))\|_1 = h + 1$, then $c_1(\phi) \geq 8$.
  \label{lemma4}
\end{lemma}
\begin{proof}
  The proof is omitted as it is similar to that of Lemma~\ref{lemma2}.
\end{proof}

\begin{lemma}
  The only embedding $\phi$ of a two-slices graph for which $\|\phi((2,1)) - \phi((2,h))\|_1 = h$ and $c_1(\phi) = 4$ is the natural embedding, up to rotation, translation and symmetry.
  \label{lemma5}
\end{lemma}
\begin{proof}
  If $\phi((2,1))$ and $\phi((2,h))$ are on the same line or column, the reasoning is very similar to that of Theorem~\ref{chap3:theorem-grid}.

  We already have $\delta((2,1),(2,h)) = 2$. So to achieve $c_1(\phi) = 4$, we must have $(1,1)$ and $(1,h)$ not embedded on a shortest (Manhattan) path between the embedded versions of $(2,1)$ and $(2,h)$. Their distance is thus $h+2$.
\end{proof}

\begin{lemma}
  The only optimal embedding of a two-slices graph is the natural embedding, up to rotation, translation and symmetry.
  \label{lemma6}
\end{lemma}
\begin{proof}
  First observe that any embedding for which $\delta((2,1),(2,h)) \geq 3$ is not optimal. We conclude with Lemmas 1 to 5.
\end{proof}

Now we can derive the main result of the subsection:
\begin{theorem}
  The only optimal embedding of a quasi grid graph is the natural embedding, up to rotation, translation and symmetry.
\end{theorem}
\begin{proof}
  Consider the missing edge in the quasi grid graph is at column $j$. Now we can discuss the sum in $c_1$. For couple of vertices one of which is not on column $j-1$, $j$ or $j+1$, observe that the natural embedding has cost 0. For the remaining couple of vertices, we discuss on the rows: if both rows are above or both rows are below the missing edge, cost is 0. For the remaining cases, we use Lemma~\ref{lemma6} to prove the natural embedding is the only one to minimize the cost.
\end{proof}

\subsection{Optimization methodology}

Using a bruteforce approach to find optimal embeddings is clearly impossible for graphs of reasonable order. In order to find a proxy to an optimal embedding, we propose to use the combination of gradient descent and barrier~\citep{murray2010algorithm} methods. We start with a random projection in an hypercube of $\mathbb{R}^d$. The gradient descent aims at minimizing the weighted sum of the cost of the embedding and a penalty of how far away it is from $\mathbb{Z}^d$. The barrier method consists in smoothly modifying the scaling of the two parts of the cost by making use of two scaling parameters $\beta$ and $\gamma$. As a result, at the first iterations the optimization is performed in $\mathbb{R}^d$ and we only aim at minimizing the cost, whereas in the last iterations we enforce the solution to be in $\mathbb{Z}^d$. In the experiments, we use $\beta = 10^{-6}$ and $\gamma = 1.03$.

An overview of the algorithm is:~\begin{algorithm}[ht]
    \textbf{Data}: Graph $G$, dimension $d$, scaling factor $\alpha$. \\
  $\phi_0 \leftarrow \text{random embedding}$\\
  $\beta_0 \leftarrow \beta$
  \begin{algorithmic}
  \FOR{i \text{ in } (1,\dots,K)}
  \STATE $\beta_i \leftarrow \gamma\beta_{i-1}$
  \STATE  $\phi_i \leftarrow GradMin_{\phi}{
    \left(\frac{c_\alpha(\phi) + \beta_i\left[\sum_{v}{d_1(\phi(v),\mathbb{Z}^d)}\right]}{1+\beta_i}, \phi_{i-1}\right)}$    
  \ENDFOR
  \end{algorithmic}
  \caption{Proposed optimization methodology, $d_1(\phi(v),\mathbb{Z}^d)$ denotes the Manhattan distance between $\phi(v)$ and $\mathbb{Z}^d$, $GradMin_\phi(c(\phi),\phi_0)$ denotes a gradient descent algorithm with parameter $\phi$ starting from $\phi=\phi_0$ and aiming at minimizing $c(\phi)$.}
  \label{chap3:algo-embeddings}
\end{algorithm}

A depiction of different steps in the algorithm is presented in Figure~\ref{chap3:embedding-illustration}. On the first line we consider a 2D grid graph, whereas on the second line we represent a random geometric graph. As we can see, the embedding at the end of the first gradient descent is already the natural embedding for the grid graph. This is because of the choice of the Manhattan distance in the definition of $c_\alpha$. To the contrary, the embedding obtained at the end of the first gradient descent is not aligned with $\mathbb{Z}^2$ in the case of the random geometric graph.

\begin{figure}[ht]
    \begin{center}
      \begin{tabular}{m{2cm}ccc}
      & Initial embedding & After first descent & Final embedding\\
      \vspace{-3.5cm}Grid graph (10x10 vertices)& \inputtikz{chapter3/tikz/gridstart}& \inputtikz{chapter3/tikz/gridend} & \inputtikz{chapter3/tikz/gridend}\\
      \vspace{-3.5cm}Random geometric graph (200 vertices, radius of 0.2)& \inputtikz{chapter3/tikz/geometricstart}& \inputtikz{chapter3/tikz/geometricmiddle}& \inputtikz{chapter3/tikz/geometricend}
    \end{tabular}
    \end{center}
  \caption{Illustration of successive steps in the optimisation procedure from Algorithm~\ref{chap3:algo-embeddings}. Left column is initial random embedding, middle column is after the first gradient descent, and right column at the end of the process. A parameter of $\alpha=1$ was used for the grid graph and $\alpha=2$ for the random geometric graph. Figure extracted from~\citep{grelier2018graph}.}
    \label{chap3:embedding-illustration}
  \end{figure} 
  
  \subsection{Experiments and results}

  In terms of experiments, we first compare costs of different methods for finding an embedding of grid graphs. We compare our proposed method with: a) a random embedding and b) an embedding obtained by considering the two eigenvectors associated with the smallest nonzero eigenvalues of the Laplacian of the graph. Note that for each method we choose the value of $\alpha$ that minimizes the cost.
  In the next experiment, we look at the effect of removing some of the edges in a grid graph with parameters $l,h = 10$ in terms of the distance between the obtained embedding and the natural one. Both results are summarized in Figure~\ref{chap3:emb-comp}.
  
  \begin{figure}[ht]
    \begin{center}
      \begin{subfigure}[ht]{.48\linewidth}
        \centering
        \begin{adjustbox}{max width=\linewidth}
          \inputtikz{chapter3/tikz/noisygraph}
        \end{adjustbox}
    \end{subfigure}
    \begin{subfigure}[ht]{.48\linewidth}
        \centering
        \begin{adjustbox}{max width=\linewidth}
          \inputtikz{chapter3/tikz/costs}
        \end{adjustbox}
      \end{subfigure}        
        \caption{Comparison of embedding costs obtained by various methods (right) and evolution of the distance between a noisy grid graph embedding found using Algorithm 1 and its natural embedding (left). Figure extracted from~\citep{grelier2018graph}.}
        \label{chap3:emb-comp}
    \end{center}
\end{figure}
  
  
In Figure~\ref{chap3:emb-compeigen}, we compare the eigenvectors/Fourier modes associated with the first nonzero eigenvalues/frequencies on a random geometric graph for a spectral definition based on the Laplacian and our proposed graph-projected approach. We can clearly see the interest of our proposed method in such a case where the underlying 2D structure is very important during the creation of the graph.

\begin{figure}[ht]
    \begin{center}
        \begin{tabular}{cc}
            \inputtikz{chapter3/tikz/geometricfirst} & \inputtikz{chapter3/tikz/geometricsecond} \\
            \inputtikz{chapter3/tikz/geometricfourier1} & \inputtikz{chapter3/tikz/geometricfourier2}
        \end{tabular}
        \caption{Depiction of the first eigenvectors/Fourier modes (associated with the lowest nonzero eigenvalues/frequencies) of a random geometric graph. First line corresponds to the classical graph signal processing definition (using the Laplacian), and second line to the proposed embedding. Best viewed in color. Figure extracted from~\citep{grelier2018graph}.}
        \label{chap3:emb-compeigen}
    \end{center}
\end{figure}
  
  
Finally, we compare our method against CNNs and graph CNNs in regular 2D grids and irregular 3D grid scenarios. In Table~\ref{cifar-table} we compare the performance of convolutional neural networks using our methodology with spectral solutions on the CIFAR-10 dataset an image dataset (2D grid).  Our method is able to use the same architecture as a classic CNN, while~\citep{defferrard2016convolutional} and~\citep{lassance2018matching} use a comparable but not equal architecture (c.f., Section~\ref{chap4:classify_graph_signals}). Considering data augmentation, random crops are used for all methods but~\citep{lassance2018matching}, which uses a method that approximates random crops using translations learned from the graph.
  
  \begin{table}[ht]
    \begin{center}
    \centering
    \caption{CIFAR-10 test set accuracy comparison table. Table extracted from~\citep{grelier2018graph}.}
    
    \label{cifar-table}
    \begin{tabular}{|c|c||m{1.8cm}|c|c|c|}
      \multicolumn{3}{c|}{}&Spectral&\multicolumn{2}{c|}{Nonspectral}\\
    \hline
    MLP~\citep{lin15withoutconvolution}       & CNN                     & Support  & \citep{defferrard2016convolutional} & Section~\ref{chap4:classify_graph_signals}~\citep{lassance2018matching} & Proposed~\citep{grelier2018graph} \\ \hline
    \multirow{2}{*}{78.62\%} & \multirow{2}{*}{92.73\%} & Grid & 84.41\%                            & 92.81\%             & 92.73\%  \\ \cline{3-6}
                             &                          & Covariance graph &------                             & 91.07\%             & 89.25\%  \\ \hline
    \end{tabular}
    \end{center}
\end{table}  
  
  For the irregular 3D grid scenario we use the PINES dataset, which consists of fMRI scans on 182 subjects, during an emotional picture rating task~\citep{chang2015sensitive}. We use the same methods from~\citep{lassance2018matching} to generate an irregular 3D grid. The final volumes used for classification contain 369 signals for each subject and rating. We used a shallow network for the classification task. The results are presented on Table~\ref{iaps-table}. We show that the proposed
  method is competitive with existing methods.
  
  
\begin{table}[ht]
    \centering
    \caption{PINES fMRI dataset accuracy comparison table. Results are presented using the mean over 10 tests. CNNs use a 9x9x9 filter size. Table extracted from~\citep{grelier2018graph}.}
    \label{iaps-table}
    \begin{tabular}{|l||c|c||c|c|c|}
    \hline
    \multicolumn{1}{|l||}{Graph} & \multicolumn{2}{c||}{None} & \multicolumn{3}{c|}{Neighborhood Graph}     \\ \hline
    Method                      & Dense & CNN & \citep{defferrard2016convolutional} & Section~\ref{chap4:classify_graph_signals}~\citep{lassance2018matching} & Proposed~\citep{grelier2018graph}                  \\ \hline
    Accuracy                    & $82.62\%$ & \textbf{$85.47\%$} & $82.80\%$ & $85.08\%$ & $84.78\%$ \\ \hline
    \end{tabular}
    \end{table}

We introduced an alternative definition of the Fourier transform on a graph. In the case of graphs obtained by a sampling of a regular metric space, we believe the proposed method can lead to better definition of Fourier modes and associated operators. This is supported by the experiments using convolutional neural networks.

In our experiments, finding Fourier modes for graphs containing up to a few thousands of vertices can be performed in a few minutes on a modern computer, thus requiring a time similar to that of finding eigenvectors and eigenvalues of the corresponding Laplacian matrix. It would be interesting to stress the interest of the proposed method for other graph signal uses. Also we consider running experiments on highly irregular graphs. In the next Section we are going to introduce graph filters that based on the GFT aim at reproducing traditional signal processing filters in the graph domain.

==> chapter3/tikz/noisygraph.tex <==
\begin{tikzpicture}
    \begin{axis}[
      xlabel=Probability of missing edges,
      ylabel=$c_\alpha/n^2$,
      %legend pos=north west
      ]
        \addplot table {chapter3/embedding/resloss.txt};
    \end{axis}
\end{tikzpicture}


==> notation.tex <==
\chapter*{Notation}
\label{notation}


\typeout{START_CHAPTER "notation" \theabspage}

% Sometimes we have to include the following line to get this section
% included in the Table of Contents despite being a chapter*
\addcontentsline{toc}{chapter}{Notation}
This section provides a concise reference describing notation used throughout this
document. For standardization we follow the notations from~\citep{dlbook}.

\vspace{\notationgap}
% Need to use minipage to keep title of table on same page as table
\begin{minipage}{\textwidth}
% This is a hack to put a little title over the table
% We cannot use "\section*", etc., they appear in the table of contents.
% tocdepth does not work on this chapter.
\centerline{\bf Numbers and Arrays}
\bgroup
% The \arraystretch definition here increases the space between rows in the table,
% so that \displaystyle math has more vertical space.
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
%$\displaystyle \ra$ & A scalar random variable\\
%$\displaystyle \rva$ & A vector-valued random variable\\
%$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\index{Scalar}
\index{Vector}
\index{Matrix}
\index{Tensor}
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\egroup
\index{Scalar}
\index{Vector}
\index{Matrix}
\index{Tensor}
\index{Graph}
\index{Set}
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Linear Algebra Operations}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle \mA^\top$ & Transpose of matrix $\mA$ \\
$\displaystyle \mA \odot \mB $ & Element-wise (Hadamard) product of $\mA$ and $\mB$ \\
% Wikipedia uses \circ for element-wise multiplication but this could be confused with function composition
\end{tabular}
\egroup
\index{Transpose}
\index{Element-wise product|see {Hadamard product}}
\index{Hadamard product}
\end{minipage}

%\vspace{\notationgap}
%\begin{minipage}{\textwidth}
%\centerline{\bf Calculus}
%\bgroup
%\def\arraystretch{1.5}
%\begin{tabular}{cp{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
%$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
%$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
%$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
%$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
%$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
%$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
%$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
%$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
%$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
%\end{tabular}
%\egroup
%\index{Derivative}
%\index{Integral}
%\index{Jacobian matrix}
%\index{Hessian matrix}
%\end{minipage}

%\vspace{\notationgap}
%\begin{minipage}{\textwidth}
%\centerline{\bf Probability and Information Theory}
%\bgroup
%\def\arraystretch{1.5}
%\begin{tabular}{cp{3.25in}}
%$\displaystyle \ra \bot \rb$ & The random variables $\ra$ and $\rb$ are independent\\
%$\displaystyle \ra \bot \rb \mid \rc $ & They are conditionally independent given $\rc$\\
%$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
%$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
%a variable whose type has not been specified\\
%$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
%$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
%$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
%$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
%$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
%$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
%$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
%over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
%\end{tabular}
%\egroup
%\index{Independence}
%\index{Conditional independence}
%\index{Variance}
%\index{Covariance}
%\index{Kullback-Leibler divergence}
%\index{Shannon entropy}
%\end{minipage}

\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
%$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
%$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$. Also known as the output of $\text{ReLU}(x)$\\
$\displaystyle \classifier$ & A classifier\\
$\displaystyle \featureextractor$ & A feature extractor\\
%$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
%\index{Sigmoid}
%\index{Softplus}
\index{Norm}
\end{minipage}

Sometimes we use a function $f$ whose argument is a scalar but apply
it to a vector, matrix, or tensor: $f(\vx)$, $f(\mX)$, or $f(\tX)$.
This denotes the application of $f$ to the
array element-wise. For example, if $\tC = \sigma(\tX)$, then $\etC_{i,j,k} = \sigma(\etX_{i,j,k})$
for all valid values of $i$, $j$ and $k$.


\vspace{\notationgap}
\begin{minipage}{\textwidth}
\centerline{\bf Datasets and Distributions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{cp{3.25in}}
%$\displaystyle \pdata$ & The data generating distribution\\
%$\displaystyle \ptrain$ & The empirical distribution defined by the training set\\
$\displaystyle \sX$ & A set of training examples\\
$\displaystyle \vx^{(i)}$ & The $i$-th example (input) from a dataset\\
$\displaystyle y^{(i)}\text{ or }\vy^{(i)}$ & The target associated with $\vx^{(i)}$ for supervised learning\\
$\displaystyle \mX$ & The $m \times n$ matrix with input example $\vx^{(i)}$ in row $\mX_{i,:}$\\
\end{tabular}
\egroup
\end{minipage}

\clearpage

\typeout{END_CHAPTER "notation" \theabspage}


==> q.tex <==
\def \tikzexternallastkey {8841247AFA29477F4494BC249E0B8DF9}%

